Automated DevOps Pipeline Generation for Code Repositories using Large Language Models

Automating software development processes through the orchestration of GitHub Action workflows has revolutionized the efficiency and agility of software delivery pipelines. This paper presents a detailed investigation into the use of Large Language Models (LLMs) specifically, GPT 3.5 and GPT 4 to generate and evaluate GitHub Action workflows for DevOps tasks. Our methodology involves data collection from public GitHub repositories, prompt engineering for LLM utilization, and evaluation metrics encompassing exact match scores, BLEU scores, and a novel DevOps Aware score. The research scrutinizes the proficiency of GPT 3.5 and GPT 4 in generating GitHub workflows, while assessing the influence of various prompt elements in constructing the most efficient pipeline. Results indicate substantial advancements in GPT 4, particularly in DevOps awareness and syntax correctness. The research introduces a GitHub App built on Probot, empowering users to automate workflow generation within GitHub ecosystem. This study contributes insights into the evolving landscape of AI-driven automation in DevOps practices.

==> secs/discussion.tex <==
\bowen{add the additional exp about ``add dependency yields worse result''}

The conducted ablation study aimed to assess the impact of different contextual inputs on the performance of GPT-4 in generating GitHub Action Workflows. The three prompt settings employed were (1) Repository structure & dependency list, (2) Only Repository structure, and (3) Only Dependency list.

In Table \ref{tab:discussion_devopsaware}, the comparison of DevOps Aware Scores across the different prompt settings revealed intriguing insights. Contrary to our initial hypothesis, the inclusion of dependencies did not significantly enhance the performance of GPT-4. The scores for scenarios with additional context (Repository structure + Dependency list) and those with only the Repository structure were comparable, with scores of 0.5 and 0.53, respectively. Interestingly, providing only the Dependency list resulted in a slightly lower score of 0.46. This suggests that, in our experimentation, the versioning information conveyed by project dependencies did not substantially contribute to the improvement of workflow generation.



\begin{table}[h]
\caption{Comparison of DevOps Aware Score for ablation study}
\label{tab:discussion_devopsaware}
\begin{tabular}{cc}
 \toprule
Languages  & GPT 4\\
\midrule
Repository structure + Dependency list       &     0.5   \\
Only Repository structure        &    0.53   \\
Only Dependency list       &     0.46  \\
\bottomrule
\end{tabular}
\end{table}
Further analysis, presented in Table \ref{tab:discussion_syntax}, focused on the Valid Syntax percentage across the same prompt settings. Surprisingly, the results indicated a negligible difference in syntax validity among the three scenarios. Both Repository structure settings and the Dependency list setting demonstrated a high syntax validity percentage, with minimal variations at 96.90\% and 96.88\%, respectively. This implies that GPT-4 maintained consistent syntax generation capabilities across different contextual inputs.
\begin{table}[h]
\caption{Comparison of Valid Syntax percentage for ablation study}
\label{tab:discussion_syntax}
\begin{tabular}{cc}
 \toprule
Languages  & GPT 4\\
\midrule
Repository structure + Dependency list       &     96.90 \%   \\
Only Repository structure        &    96.90 \%   \\
Only Dependency list       &     96.88 \% \\
\bottomrule
\end{tabular}
\end{table}

In conclusion, the results suggest that, for the specific task of GitHub Action Workflow generation, the inclusion of additional context in the form of project dependencies did not yield a substantial improvement. On the contrary, the study underscores the importance of the repository structure as a critical factor influencing the generation of effective workflows. Therefore, when leveraging GPT-4 for GitHub Action Workflow generation, prioritizing information related to the repository structure in the input context is recommended for optimal performance.
